Spatial Network Calculus and Performance Guarantees in Wireless Networks

This work develops a novel approach toward performance guarantees for all links in arbitrarily large wireless networks. It introduces a spatial network calculus, consisting of spatial regulation properties for stationary point processes and the first steps of a calculus for this regulation, which can be seen as an extension to space of the classical network calculus. Specifically, two classes of regulations are defined: one includes ball regulation and shot-noise regulation, which are shown to be equivalent and upper constraint interference; the other one includes void regulation, which lower constraints the signal power. These regulations are defined both in the strong and weak sense: the former requires the regulations to hold everywhere in space, whereas the latter only requires the regulations to hold as observed by a jointly stationary point process. Using this approach, we derive performance guarantees in device-to-device, ad hoc, and cellular networks under proper regulations. We give universal bounds on the SINR for all links, which gives link service guarantees based on information-theoretic achievability. They are combined with classical network calculus to provide end-to-end latency guarantees for all packets in wireless queuing networks. Such guarantees do not exist in networks that are not spatially regulated, e.g., Poisson networks.

==> generic_g_reg.tex <==

% Let $\Phi$ be a stationary point process and $\Phi_i,~i=1,...,n$ be a family of stationary point processes on $\mathbb{R}^2$, defined on the probability space $(\Omega,\mathcal{A},\mathbb{P})$. The following properties hold.  
% \begin{itemize}
%  \item {(Superposition)} If $\Phi_i$ is $g_i$-ball regulated, $i=1,...,n$, then the superposition  $\bigcup_{i=1}^{n}\{\Phi_i\}$ is $\sum_{i=1}^{n}g_i$-ball regulated. 
% \item {(Thinning)}
% If $\Phi$ is $g$-ball regulated, then $\Phi$ is $g$-ball regulated after an arbitrary thinning. 
% \item {(Displacement)} Let $\Tilde\Phi \triangleq \{x\in\Phi\colon x+V_x\}$ be a displaced point process of $\Phi$, where ${\{V_x\}}_{x\in\Phi}$ is a set of bounded random vectors preserving stationarity. If $\Phi$ is strongly $g$-ball regulated with $g(r)\sim \nu r^2$ as $r\to\infty$, then $\Tilde\Phi$ is $(\sigma,\rho,\nu)$-ball regulated for some $\sigma,\rho$. 
% \end{itemize}


==> gg1.tex <==


\subsubsection{Stochastic Bounds on Latency in Queues - Dipole Case}
The aim of this subsection is to illustrate the stochastic bounds that can be obtained
on queuing latency by spatial regulation alone, i.e., in the absence of time
regulation and in the presence of fading with short coherence times.
The illustration features a dipole type device to device network with Rayleigh fades where
each dipole is equipped with an infinite buffer FIFO queue.
Time is slotted. The packet arrival process in each queue is i.i.d. over time slots and the number of
arrivals of packets in a time slot has the distribution $A$ over the integers.
There is hence no time regulation on the input point processes.
The packet head of a given queue at a given time slot is successfully transmitted (served) if  
the SINR at that location and at that time exceeds the threshold $\theta$.
If it is the case, the packet leaves. Otherwise it stays head of the line and tries again next slot
until its transmission succeeds. 
The simplest scenario is that where the slot durations are of the order of the coherence
time of the fades. In this case, in each queue, the fades experienced 
in different time slots are i.i.d.  
In the Rayleigh fade case, the conditional probability of success in the typical queue given the transmitter
point process is bounded from below by the constant given in Theorem 5.9.
Hence, in each queue, the stationary latency is stochastically bounded from above
by that in a discrete time queue with i.i.d. arrivals with distribution $A$ and i.i.d.
Bernoulli service process with constant probability of success $p_\theta$. 
The distribution of the stationary queue size and of the latency in such queues has
been extensively studied using generating function techniques and is known in closed form
in function of $A$ and $p_\theta$ \cite{bruneel1993performance}.

The results can easily be extended to more subtle scenarios (e.g. mixing Markov evolution
of the fades over time slots in place of than i.i.d. assumptions) as well as to any of the other
network settings discussed in this paper. 
